KernelGPT: Enhanced Kernel Fuzzing via Large Language Models

Bugs in operating system kernels can affect billions of devices and users all over the world. As a result, a large body of research has been focused on kernel fuzzing, i.e., automatically generating syscall (system call) sequences to detect potential kernel bugs or vulnerabilities. Kernel fuzzing aims to generate valid syscall sequences guided by syscall specifications that define both the syntax and semantics of syscalls. While there has been existing work trying to automate syscall specification generation, this remains largely manual work, and a large number of important syscalls are still uncovered. In this paper, we propose KernelGPT, the first approach to automatically synthesizing syscall specifications via Large Language Models (LLMs) for enhanced kernel fuzzing. Our key insight is that LLMs have seen massive kernel code, documentation, and use cases during pre-training, and thus can automatically distill the necessary information for making valid syscalls. More specifically, KernelGPT leverages an iterative approach to automatically infer the specifications, and further debug and repair them based on the validation feedback. Our results demonstrate that KernelGPT can generate more new and valid specifications and achieve higher coverage than state-of-the-art techniques. So far, by using newly generated specifications, KernelGPT has already detected 24 new unique bugs in Linux kernel, with 12 fixed and 11 assigned with CVE numbers. Moreover, a number of specifications generated by KernelGPT have already been merged into the kernel fuzzer Syzkaller, following the request from its development team.

==> 3-approach-old.tex <==
\begin{figure*}[t]
    \includegraphics[width=0.95\textwidth]{figures/overview.pdf}
    \caption{Overview of \tech\chenyuan{more general, value, type, dependency recovery}}
    \label{fig:overview}
\end{figure*}

Figure~\ref{fig:overview} presents the overview of \tech, which utilizes the code extractor and analysis \llm{} to automatically generate specifications for enhancing kernel fuzzing.
While the approach is general to various syscalls, \tech targets those for drivers and sockets, given the fact that they constitute about 70\% LoC in the kernel~\cite{bursey2024syzretrospector}.
\tech takes the kernel codebase and located device and socket operation handlers as input and operates through three automated phases: \handlerSection \circled{1}, Specification Generation \circled{2}, and Specification Validation and Repair \circled{3}.

Initially, \tech identifies the driver (or socket) by employing \llm{s} to infer the device name (or the domain, type, and protocol) and its initialization specification, using the details of the operation handler and its usage (\S~\ref{subsec:driver-detect} \circled{1}).
Subsequently, \tech determines the command values, argument types, and type definitions for describing the syscalls associated with the driver and socket.
In doing so, \tech utilizes the relevant source code from the kernel codebase to guide the \llm{s} in their analysis in a novel iterative way.
If essential information for inference is missing, the analysis \llm{} is instructed to indicate what additional information is required, which is then gathered and presented for analysis in the following step (\S~\ref{subsec:spec-generation} \circled{2}).
Lastly, \tech validates the generated specifications. If errors are found, it attempts to repair the descriptions by consulting the \llm{s} with the error messages (\S~\ref{subsec:spec-repair} \circled{3}).

We assume that the locations for the driver and socket operation handlers are known for \tech since they can be identified by simple yet general patterns.
Therefore, we use a specialized code parser implemented with \llvm~\cite{llvm} to search the kernel codebases to pinpoint instances where the operation handler structs are initialized with \CodeIn{ioctl} handler functions.
More specifically, we search for initialization instances of the \CodeIn{ioctl} or \CodeIn{unlocked\_ioctl} fields within the operation handler structs.
For instance, the device mapper driver shown in Figure~\ref{fig:dm-ctl-example-a} initiates the \CodeIn{unlocked\_ioctl} field in \CodeIn{\_ctl\_fops} structure by using \CodeIn{dm\_ctl\_ioctl} function.
We label \CodeIn{\_ctl\_fops} as the device operation handler and extract \CodeIn{dm\_ctl\_ioctl} for analyzing \CodeIn{ioctl} descriptions.
Notably, the focus of \tech is on the inference from the source code to descriptions, rather than locating the operation handlers.
Hence, we employ a straightforward pattern-searching method to find the device and socket operations.

Considering \CodeIn{ioctl} as one of the most complex syscalls, we use it as the case study to illustrate the process of syscall description generation in the subsequent subsections.
The support for other syscalls is generally similar, if not simpler.


%





\subsection{\handlerSection}
\label{subsec:driver-detect}

%

To deduce the device driver name or socket domain, our approach begins with locating the references to its operation handler, utilizing the kernel code extractor.
Following this, we employ the usage information to guide the \llm{s} in the inference.
To enhance the accuracy, we apply few-shot in-context learning techniques~\cite{fewshot}, crafting specific prompts that aid the model in better understanding the nuances.

Figure~\ref{fig:step0} illustrates the example prompt used for inferring the driver device name.
It includes the instruction, the source code of the operation handler, and its usage, concluding with the specification that is to be generated by \llm{s}.
We anticipate that the \llm{s} will not only determine the device name (\CodeIn{DEVICE NAME} in Figure~\ref{fig:step0}) but also analyze the initialization descriptions associated with the device (\CodeIn{INITIALIZATION}).
Typically, the initialization is described with the syscall \CodeIn{openat} or \CodeIn{syz\_open\_dev} for most drivers.
Referring back to the device mapper driver, the operation handler \CodeIn{\_ctl\_fops} is utilized during the initialization of \CodeIn{struct miscdevice \_dm\_misc}, as shown in Figure~\ref{fig:step0}.
After analyzing this source code usage, \llm{s} can determine the correct device name, in this case, \CodeIn{mapper/control}, based on the \CodeIn{nodename} field within the \CodeIn{miscdevice} struct.
Since \llm{s} have assimilated such knowledge during their pre-training phase, they are capable of inferring the correct device name and initialization specification with the appropriate reference information.

Additionally, we infer the socket handler using a prompt template similar to that for the driver, as illustrated in Figure~\ref{fig:socket-prompt}. The key distinction lies in the requirement to infer the domain, type, and protocol for sockets, in contrast to deducing only the device name for drivers.
Nevertheless, akin to the approach for drivers, we provide the source code of the operation handler and its usage with \llm{s} to analyze the socket information and its initialization description.




\begin{figure}
    \centering
        \includegraphics[width=0.95\linewidth]{figures/step0-prompt.pdf}
    \caption{Prompt for driver handler inference}
    \label{fig:step0}
\end{figure}

\begin{figure}[t]
    \centering
        \includegraphics[width=0.95\linewidth]{figures/step0-socket.pdf}
    \caption{Prompt for socket handler inference}
        \label{fig:socket-prompt}
\end{figure}

%




\subsection{Specification Generation}
\label{subsec:spec-generation}

In this phase, we generate the descriptions of syscalls related to the driver or socket by leveraging \llm{s} to analyze their implementation source code.
Initially, we identify the syscall handler functions, such as \CodeIn{ioctl} and \CodeIn{setsockopt}, from their respective operation.
To enhance the performance of \llm{s}, we segment the process into three distinct stages: deducing the command value, identifying the argument type, and defining the type.
While these stages are applicable to various syscalls, certain simple ones, like \CodeIn{sendto}, may not require the deduction of a command value.
This structured approach enables \llm{s} to concentrate on one specific aspect at each stage, thereby improving efficiency and focus.
Similar to the device name inference process, we utilize in-context few-shot prompting~\cite{fewshot} at each stage of the specification generation. By providing relevant examples, we aim to enhance \llm{s}' comprehension of the task and the expected output format.

\begin{algorithm}[t]
\small
\caption{Iterative Analysis by \llm{s}}
\label{algo:analyze}
\DontPrintSemicolon
\SetKwProg{Fn}{Function}{:}{}

\SetKwData{relatedsrc}{relatedCode}
\SetKwData{usage}{usageInfo}
\SetKwData{step}{step}
\SetKwData{result}{result}
\SetKwData{success}{successResult}
\SetKwData{unknown}{unknown}
\SetKwData{id}{id}
\SetKwData{relatedfunc}{funcs}
\SetKwData{relatedtype}{types}
\SetKwData{res}{res}
\SetKwData{prompt}{prompt}

\SetKwData{maxiter}{MAX\_ITER}
\SetKwFunction{QueryLLM}{\textbf{QueryLLM}}
\SetKwFunction{FindCode}{\textbf{ExtractCode}}
\SetKwFunction{update}{\textbf{Update}}
\SetKwFunction{Analyze}{\textbf{Analyze}}
\SetKwFunction{GenPrompt}{\textbf{GenPrompt}}

\Fn{\Analyze{\relatedsrc, \usage, \step}}{
\If{\step > \maxiter}{
    \Return{$\emptyset$}\; \label{line:max-iter}
}
\textit{\scriptsize\color{applegreen}\# Prepare the prompt with few-shot examples}\;
\prompt $\leftarrow$ \GenPrompt(\relatedsrc, \usage) \; \label{line:prompt-gen}
\textit{\scriptsize\color{applegreen}\# Query \llm{} to analyze the source code and identify the unknown}\;
\success, \unknown $\leftarrow$ \QueryLLM(\prompt)\; \label{line:query}
\For{$(\id, \usage) \in \unknown$}{\label{algo:sample-start}
    \textit{\scriptsize\color{applegreen}\# Extract the code based on the unknown identifier}\;
    \relatedsrc $\leftarrow$ \FindCode(\id)\label{line:extract}\;
    \textit{\scriptsize\color{applegreen}\# Recursively analyze the missing source code}\;
    \res $\leftarrow$ \Analyze(\relatedsrc, \usage, $\step+1$)\; \label{line:next-step}
    \textit{\scriptsize\color{applegreen}\# Update with the result analyzed for the unknown}\;
    \update(\success, \res)\;
}\label{algo:sample-end}
\Return{$\success$}\;
}

\end{algorithm}

We develop a novel iterative method to utilize and improve the code analysis capabilities of \llm{s}, which is motivated by two primary factors.
Firstly, despite state-of-the-art \llm{s} such as \gpt{4} supporting a context size of 128K~\cite{gpt4-turbo}, it remains impractical to provide \llm{s} with the entirety of the source code related to a driver or socket.
Secondly, our goal is to deduce the command value and argument type for the syscall, and not all the code or helper functions within the syscall handler are pertinent to this objective.
Recognizing that some parts may not contribute to our aim, we have devised a strategy where \llm{s} analyze the kernel code recursively, as shown in Algorithm~\ref{algo:analyze}.
Firstly, we generate a few-shot example prompt with the source code related to the target and its usage information (Line~\ref{line:prompt-gen}).
Then, \llm{s} are queried to infer the descriptions and pinpoint any function or type that is missing yet essential for inference in the \CodeIn{unknown} set (Line~\ref{line:query}).
For each unknown candidate, we extract the source code based on its identifier (Line~\ref{line:extract}), which is supplied to \llm{s} along with its usage information in the subsequent step for further analysis (Line~\ref{line:next-step}).
The analysis concludes and outputs the results either when no unknown elements are detected or when the iteration count exceeds \CodeIn{MAX\_ITER} (Line~\ref{line:max-iter}).
Importantly, the entire analysis process is fully automated, steered by the unknown information provided by \llm{s}.







\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\columnwidth]{figures/step1-prompt.pdf}
    \caption{Prompt for command value analysis}
    \label{fig:step1}
\end{figure}

\subsubsection{Command Value}

We use an iterative prompting strategy for analyzing command values, as depicted in Figure~\ref{fig:step1}.
In addition to the instruction, this prompt includes the source code of functions relevant to the inference task.
This encompasses the syscall handler function and any associated helper functions pertinent to command value analysis.
The expected output from \llm{s} is the set of successfully inferred command values.
If the logic for checking command values is delegated to another function not presented to \llm{s}, we instruct \llm{s} to list the name and invocation details of this ``missing'' dispatched function (the \CodeIn{UNKNOWN} field).
Furthermore, code snippets that reference the command variables are also included.
Should \llm{s} identify any unknown command values, \tech proceeds to analyze the newly identified dispatched function, incorporating their usage information from the previous step.
In essence, the output from the \CodeIn{UNKNOWN} field of the previous step serves as a reference for guiding subsequent steps.

Figure~\ref{fig:step1} presents the first two steps of command value analysis for the device mapper driver.
The \CodeIn{dm\_ctl\_ioctl} handler, registered as the \CodeIn{ioctl} handler, offloads its entire functionality to another function, \CodeIn{ctl\_ioctl}.
As a result, after examining \CodeIn{dm\_ctl\_ioctl}, \llm{s} are unable to deduce any command values and designate \CodeIn{ctl\_ioctl} as the absent function.
Subsequently, \tech extracts the source code for \CodeIn{ctl\_ioctl} and, together with the unknown information returned by the first step, re-queries \llm{s}.
In the second round, \llm{s} successfully identifies one command value, \CodeIn{DM\_VERSION}, while other values related to the function \CodeIn{lookup\_ioctl} remain undetermined.
Thus, \llm{s} report \CodeIn{DM\_VERSION} as one command value and \CodeIn{lookup\_ioctl} as the missing function, which will be analyzed in the next step to infer more command values.





\subsubsection{Argument Type}

\begin{figure}
    \centering
    \includegraphics[width=0.95\columnwidth]{figures/step2-prompt.pdf}
    \caption{Prompt for argument type inference}
    \label{fig:step2}
\end{figure}

After determining the command value, the subsequent stage involves analyzing the argument type, as depicted in the prompt shown in Figure~\ref{fig:step2}.
The initial information for this inference, derived from the command value inference stage, includes relevant functions and code snippets demonstrating the argument's usage.
\tech then extracts the source code for these related functions and presents them to \llm{s}, which are tasked with identifying the argument type.
If the code logic that determines the argument type is delegated to another function, the type will still be marked as \CodeIn{UNKNOWN}.
In such instances, \tech continues its analysis, leveraging the new information provided by \llm{s}.

Figure~\ref{fig:step2} shows an example of argument inference for the \CodeIn{DM\_REMOVE\_ALL} command value in the device mapper driver.
In the preceding step, \llm{s} identify the function associated with this argument as \CodeIn{remove\_all}, along with its usage code.
Consequently, \tech supplies \llm{s} with the source code of \CodeIn{remove\_all} to guide the argument type inference.
Analyzing its signature, \llm{s} deduce that the argument should be a pointer to the struct \CodeIn{dm\_ioctl}.
Additionally, \llm{s} place the struct \CodeIn{dm\_ioctl} in the \CodeIn{TYPES} field, setting it up for type definition analysis in the following stage.

\subsubsection{Dependency}

\chenyuan{TODO, add one more component to analyze whether the returned value of the ioctl is file descriptor or not}


\subsubsection{Type Definition}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\columnwidth]{figures/step3-prompt.pdf}
    \caption{Prompt for type definition generation}
    \label{fig:step3}
\end{figure}

Once the argument types are identified, \tech generates descriptions for them.
Figure~\ref{fig:step3} displays the prompt used in this stage.
Essentially, \tech retrieves the definition source code of the type from the \kernel codebase.
This source code is then presented to \llm{s}, tasked with creating the corresponding \syzkaller description.
In cases with a reference to a nested type within the type definition, \llm{s} are instructed to mark it as \CodeIn{UNKNOWN} in their output.
These marked types are then further analyzed in subsequent steps.

The type definition inference example depicted in Figure~\ref{fig:step3} showcases a specific case: one field of \CodeIn{PhysDevAddr\_struct} is an array composed of the struct type \CodeIn{SCSI3Addr\_struct}.
As the source code for this newly referenced struct, \CodeIn{SCSI3Addr\_struct}, is not included in the provided information, \llm{s} are expected to identify it as \CodeIn{UNKNOWN}.
This designation indicates that \CodeIn{SCSI3Addr\_struct} requires further analysis in the subsequent step.


\subsection{Specification Validation and Repair}
\label{subsec:spec-repair}

\begin{figure}
    \centering
    \includegraphics[width=0.95\columnwidth]{figures/step4-prompt.pdf}
    \caption{Prompt for specification repair}
    \label{fig:step4}
\end{figure}

In this phase, inspired by recent work on \llm-based program repair~\cite{chatrepair}, our goal is to validate the specifications generated by \tech and automatically repair the invalid ones by leveraging \llm{s}.
This step is crucial, as \llm{s} may occasionally make mistakes during the description generation process.
To address this, we utilize two tools in \syzkaller, \CodeIn{syz-extract} and \CodeIn{syz-generate}, which can validate the specifications by detecting many types of errors, including issues like undefined types, wrong macro names, and more. 
Initially, \tech uses the error messages from them to pinpoint inaccuracies in specific descriptions, effectively matching each error message to its corresponding description.
Then, for those descriptions identified with errors, \tech queries \llm{s} for correction, guided by few-shot examples.
This process, depicted in Figure~\ref{fig:step4}, involves supplying \llm{s} with the incorrect description, the associated error messages, and relevant source code from the kernel codebase to repair.
\llm{s} are then expected to output the correct descriptions.

For example, as illustrated in Figure~\ref{fig:step4}, the type description for \CodeIn{vfio\_pci\_hot\_reset\_info} is initially incorrect.
This is due to \syzlang's requirement for the length in \CodeIn{array[type, length]} to be a constant, whereas the description uses a variable \CodeIn{count} as the length.
The correct format for a variable-length array in \syzlang is simply \CodeIn{array[type]}.
By analyzing the error message ``count is unsupported on all arches'' generated by \CodeIn{syz-extract}, \llm{s} repair this issue by redefining \CodeIn{devices} as a variable-length array and specifying \CodeIn{count} as a type \CodeIn{len[devices]}, thereby aligning the description with the requirements of \syzlang.

